MALAMUTE: A Multilingual, Highly-granular, Template-free, Education-based Probing Dataset

Language models (LMs) have excelled in various broad domains. However, to ensure their safe and effective integration into real-world educational settings, they must demonstrate proficiency in specific, granular areas of knowledge. Existing cloze-style benchmarks, commonly used to evaluate LMs' knowledge, have three major limitations. They: 1) do not cover the educational domain; 2) typically focus on low-complexity, generic knowledge or broad domains, which do not adequately assess the models' knowledge in specific subjects; and 3) often rely on templates that can bias model predictions. Here, we introduce MALAMUTE, a multilingual, template-free, and highly granular probing dataset comprising expert-written, peer-reviewed probes from 71 university-level textbooks across three languages (English, Spanish, and Polish). MALAMUTE is the first education-based cloze-style dataset. It covers eight domains, each with up to 14 subdomains, further broken down into concepts and concept-based prompts, totaling 33,361 university curriculum concepts and 116,887 prompts. MALAMUTE's fine granularity, educational focus, and inclusion of both sentence-level and paragraph-level prompts make it an ideal tool for evaluating LMs' course-related knowledge. Our evaluation of masked and causal LMs on MALAMUTE shows that despite overall proficiency, they have significant gaps in knowledge when examined closely on specific subjects, hindering their safe use in classrooms and underscoring the need for further development.

==> CLM_results_table.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{1.5pt}
\tiny
% \begin{tabular}{ll|*{10}{>{\centering\arraybackslash}m{1.2cm}}}
\begin{tabular}{ll|llllllll}
\hline

\multicolumn{1}{c}{\textbf{Domain}} & \multicolumn{1}{c|}{\textbf{Subdomain}} & 

\multicolumn{8}{c}{\textbf{Causal LMs}} \\
& & \multicolumn{2}{c}{\textbf{Bloom}} & \multicolumn{2}{c}{\textbf{Mistral}} & \multicolumn{2}{c}{\textbf{Llama2}} & \multicolumn{2}{c}{\textbf{Llama3}} \\
& & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} \\
\hline

\multirow{5}{*}{Math} 
        & Prealgebra & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Elementary Algebra & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Intermediate Algebra & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & College Algebra & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Trigonometry & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Precalculus $\textcolor{purple}\star$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Calculus I $\textcolor{purple}\star$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Calculus II $\textcolor{purple}\star$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Calculus III $\textcolor{purple}\star$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Intro. Statistics & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Business Statistics $\textcolor{purple}\star$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Statistics & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Contemporary Math & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        \hline
\multirow{5}{*}{Science} 
        & Concepts of Biology & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Biology & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Microbiology & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Chemistry Atoms First & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Chemistry $\textcolor{purple}\star$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Organic Chemistry & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Anatomy & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Astronomy & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & College Physics & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Physics & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Physics I $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Physics II $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Physics III $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        \hline
\multirow{5}{*}{Humanities} 
        & U.S. History & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Writing & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Philosophy & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & World History I & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & World History II & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        \hline
\multirow{5}{*}{Business} 
        & Intro. to Business & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Financial Accounting  & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Managerial Accounting  & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Business Ethics & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Org. Behavior & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Finance & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Business Law & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Intellectual Property & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Marketing & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Management & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Economics & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Macroeconomics $\textcolor{red}\diamond$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Microeconomics $\textcolor{red}\diamond$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Entrepeneurship & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        \hline
\multirow{1}{*}{Nursing}    
        & Nutrition & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Computer \\ Science\end{tabular}} & Python Programming & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\ 
& Workplace Software & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Social \\ Sciences\end{tabular}} & American Government & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Anthropology & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Political Science & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Psychology $\textcolor{red}\diamond$ & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & Sociology & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}College \\ Success\end{tabular}}    
        & College Success & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        & College Success Concise & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] & [P1, P2, P3] \\
        \hline
        
\end{tabular}
\caption{\label{causal-lms} Causal models' accuracies (percentages) \textbf{on the English portion of the dataset}. Results are shown as [prompt 1, prompt 2, prompt 3]. Books that are also in Polish are marked with $\textcolor{red}\diamond$, where books that are also in Spanish are marked with $\textcolor{purple}\star$, and their results can be seen in Tables T1, T2. S=sentence-level prompts; P=paragraph-level prompts. }
\end{table*}


==> MLM_results_table.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{1.5pt}
\tiny
\begin{tabular}{ll|*{10}{>{\centering\arraybackslash}m{1.2cm}}}
\hline
\multicolumn{1}{c}{\textbf{Domain}} & \multicolumn{1}{c|}{\textbf{Subdomain}} & 
\multicolumn{8}{c}{\textbf{Causal LMs}} \\
& & \multicolumn{2}{c}{\textbf{BERT}} & \multicolumn{2}{c}{\textbf{DistilBERT}} & \multicolumn{2}{c}{\textbf{XLM-RoBERTa}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{SciBERT}} \\

& & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} \\
\hline


\multirow{5}{*}{Math} 
        & Prealgebra & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Elementary Algebra & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Intermediate Algebra & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & College Algebra & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Trigonometry & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Precalculus $\textcolor{purple}\star$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Calculus I $\textcolor{purple}\star$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Calculus II $\textcolor{purple}\star$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Calculus III $\textcolor{purple}\star$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Intro. Statistics & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Business Statistics $\textcolor{purple}\star$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Statistics & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Contemporary Math & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        \hline
\multirow{5}{*}{Science} 
        & Concepts of Biology & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Biology & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Microbiology & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Chemistry Atoms First & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Chemistry $\textcolor{purple}\star$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Organic Chemistry & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Anatomy & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Astronomy & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & College Physics & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Physics & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Physics I $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Physics II $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Physics III $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        \hline
\multirow{5}{*}{Humanities} 
        & U.S. History & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Writing & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Philosophy & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & World History I & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & World History II & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        \hline
\multirow{5}{*}{Business} 
        & Intro. to Business & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Financial Accounting  & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Managerial Accounting  & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Business Ethics & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Org. Behavior & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Finance & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Business Law & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Intellectual Property & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Marketing & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Management & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Economics & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Macroeconomics $\textcolor{red}\diamond$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Microeconomics $\textcolor{red}\diamond$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Entrepeneurship & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        \hline
\multirow{1}{*}{Nursing}    
        & Nutrition & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Computer \\ Science\end{tabular}} & Python Programming & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\ 
& Workplace Software & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Social \\ Sciences\end{tabular}} & American Government & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Anthropology & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Political Science & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Psychology $\textcolor{red}\diamond$ & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & Sociology & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}College \\ Success\end{tabular}}    
        & College Success & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        & College Success Concise & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] & [X,Y,Z] \\
        \hline
        
\end{tabular}
\caption{\label{causal-lms} Masked models' accuracies (percentages) \textbf{on the English portion of the dataset}. Results are shown as [top1, top5, top10]. Books that are also in Polish are marked with $\textcolor{red}\diamond$, where books that are also in Spanish are marked with $\textcolor{purple}\star$, and their results can be seen in Tables T1, T2. S=sentence-level prompts; P=paragraph-level prompts.}
\end{table*}

==> MLM_results_table_old.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{1.5pt}
\tiny

\begin{tabular}{ll|lllll}
\hline
\multicolumn{1}{c}{\textbf{Domain}} & \multicolumn{1}{c|}{\textbf{Subdomain}} & \multicolumn{5}{c}{\textbf{Masked LMs}} \\
& & \textbf{BERT} & \textbf{DistilBERT} & \textbf{XLM-RoBERTa} & \textbf{mBERT} & \textbf{SciBERT} \\
\hline


\multirow{5}{*}{Math} 
        & Prealgebra & - & - & - & - & - \\
        & Elementary Algebra & - & - & - & - & - \\
        & Intermediate Algebra & - & - & - & - & - \\
        & College Algebra & - & - & - & - & - \\
        & Trigonometry & - & - & - & - & - \\
        & Precalculus $\textcolor{purple}\star$ & - & - & - & - & - \\
        & Calculus I $\textcolor{purple}\star$ & - & - & - & - & - \\
        & Calculus II $\textcolor{purple}\star$ & - & - & - & - & - \\
        & Calculus III $\textcolor{purple}\star$ & - & - & - & - & - \\
        & Intro. Statistics & - & - & - & - & - \\
        & Business Statistics $\textcolor{purple}\star$ & - & - & - & - & - \\
        & Statistics & - & - & - & - & - \\
        & Contemporary Math & - & - & - & - & - \\
        \hline
\multirow{5}{*}{Science} 
        & Concepts of Biology & - & - & - & - & - \\
        & Biology & - & - & - & - & - \\
        & Microbiology & - & - & - & - & - \\
        & Chemistry Atoms First & - & - & - & - & - \\
        & Chemistry $\textcolor{purple}\star$ & - & - & - & - & - \\
        & Organic Chemistry & - & - & - & - & - \\
        & Anatomy & - & - & - & - & - \\
        & Astronomy & - & - & - & - & - \\
        & College Physics & - & - & - & - & - \\
        & Physics & - & - & - & - & - \\
        & Physics I $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & - & - & - & - & - \\
        & Physics II $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & - & - & - & - & - \\
        & Physics III $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & - & - & - & - & - \\
        \hline
\multirow{5}{*}{Humanities} 
        & U.S. History & - & - & - & - & - \\
        & Writing & - & - & - & - & - \\
        & Philosophy & - & - & - & - & - \\
        & World History I & - & - & - & - & - \\
        & World History II & - & - & - & - & - \\
        \hline
\multirow{5}{*}{Business} 
        & Intro. to Business & - & - & - & - & - \\
        & Financial Accounting & - & - & - & - & - \\
        & Managerial Accounting & - & - & - & - & - \\
        & Business Ethics & - & - & - & - & - \\
        & Org. Behavior & - & - & - & - & - \\
        & Finance & - & - & - & - & - \\
        & Business Law & - & - & - & - & - \\
        & Intellectual Property & - & - & - & - & - \\
        & Marketing & - & - & - & - & - \\
        & Management & - & - & - & - & - \\
        & Economics & - & - & - & - & - \\
        & Macroeconomics $\textcolor{red}\diamond$ & - & - & - & - & - \\
        & Microeconomics $\textcolor{red}\diamond$ & - & - & - & - & - \\
        & Entrepeneurship & - & - & - & - & - \\
        \hline
\multirow{1}{*}{Nursing}    
        & Nutrition & - & - & - & - & - \\
        \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Computer \\ Science\end{tabular}} & Python Programming & - & - & - & - & - \\ 
& Workplace Software & - & - & - & - & - \\
        \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Social \\ Sciences\end{tabular}} & American Government & - & - & - & - & - \\
        & Anthropology & - & - & - & - & - \\
        & Political Science & - & - & - & - & - \\
        & Psychology $\textcolor{red}\diamond$ & - & - & - & - & - \\
        & Sociology & - & - & - & - & - \\
        \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}College \\ Success\end{tabular}}    
        & College Success & - & - & - & - & - \\
        & College Success Concise & - & - & - & - & - \\
        \hline
\end{tabular}
\caption{\label{masked-lms} Models' accuracies (percentages) for Masked LMs. Books that are also in Polish are marked with $\textcolor{red}\diamond$, where books that are also in Spanish are marked with $\textcolor{purple}\star$. }
\end{table*}


==> MLM_results_table_with_scores.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{0.6pt}
\tiny
\begin{tabular}{l|*{11}{>{\centering\arraybackslash}m{1.5cm}}}
\hline
\multicolumn{1}{c|}{\textbf{Subdomain}} & 
\multicolumn{10}{c}{\textbf{Mask LMs}} \\
& \multicolumn{2}{c}{\textbf{BERT}} & \multicolumn{2}{c}{\textbf{DistilBERT}} & \multicolumn{2}{c}{\textbf{XLM-RoBERTa}} & \multicolumn{2}{c}{\textbf{mBERT}} & \multicolumn{2}{c}{\textbf{SciBERT}} \\

& \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} & \textbf{S} & \textbf{P} \\
\hline
Prealgebra & [12.1, 32.3, 42.4] & [11.9, 36.9, 47.7] & [12.5, 32.7, 43.4] & [11.6, 38.4, 48.7] & [15.8, 31.3, 41.1] & [14.9, 36.9, 46.1] & [7.7, 22.9, 31.3] & [5.7, 26.8, 37.4] & [17.5, 39.7, 50.2] & [\textbf{22.2}, \textbf{46.9}, \textbf{54.6}] \\
Elementary Algebra & [14.2, 33.3, 44.7] & [13.0, 38.6, 44.9] & [13.2, 33.8, 47.9] & [12.7, 37.7, 47.2] & [13.2, 32.4, 42.5] & [15.5, 35.8, 45.3] & [3.7, 21.9, 32.4] & [8.9, 25.0, 33.5] & [18.7, 42.5, 54.3] & [\textbf{22.2}, \textbf{44.9}, \textbf{55.4}] \\
Intermediate Algebra & [10.7, 26.3, 35.8] & [13.1, 32.4, 41.6] & [11.5, 30.0, 37.4] & [14.4, 35.5, 45.9] & [10.3, 25.5, 32.9] & [11.3, 29.4, 39.1] & [4.1, 21.8, 28.0] & [7.6, 26.3, 34.6] & [13.6, 35.0, 41.2] & [\textbf{18.7}, \textbf{44.0}, \textbf{55.0}] \\
College Algebra & [10.8, 34.0, 42.4] & [11.9, 37.8, 50.2] & [10.3, 33.5, 45.8] & [14.9, 36.8, 47.3] & [7.4, 26.6, 36.9] & [11.4, 27.9, 42.3] & [3.4, 19.2, 25.1] & [4.5, 22.9, 30.3] & [16.7, 44.8, 55.2] & [\textbf{23.4}, \textbf{49.8}, \textbf{59.2}] \\
Trigonometry & [9.2, 25.8, 33.4] & [7.8, 28.2, 35.9] & [9.5, 28.2, 35.8] & [8.7, 31.6, 41.7] & [8.9, 23.2, 31.1] & [10.2, 27.4, 36.2] & [3.4, 16.6, 22.6] & [4.1, 22.1, 27.9] & [16.6, 36.6, 45.0] & [\textbf{18.0}, \textbf{42.0}, \textbf{52.9}] \\
Precalculus & [8.6, 24.5, 30.7] & [8.8, 26.9, 34.7] & [9.0, 24.8, 33.4] & [9.7, 29.7, 39.2] & [8.3, 24.5, 32.4] & [11.1, 28.0, 37.2] & [3.7, 18.3, 26.8] & [5.3, 22.4, 29.4] & [12.9, 38.0, 45.6] & [\textbf{17.6}, \textbf{43.6}, \textbf{52.3}] \\
Calculus 1 & [16.2, 28.6, 36.4] & [14.8, 32.3, 37.6] & [14.3, 34.4, 46.8] & [18.0, 37.6, 49.7] & [11.0, 28.6, 44.2] & [18.0, 40.2, 47.1] & [10.4, 26.0, 35.7] & [11.1, 32.3, 38.6] & [20.1, 48.7, 59.1] & [\textbf{26.5}, \textbf{55.0}, \textbf{60.8}] \\
Calculus 2 & [12.4, 33.3, 41.4] & [14.1, 35.7, 42.6] & [11.9, 37.1, 44.3] & [15.6, 38.0, 48.7] & [14.3, 31.4, 41.0] & [16.3, 42.2, 48.3] & [10.0, 27.6, 33.3] & [13.7, 34.6, 38.8] & [22.4, 41.4, 49.0] & [\textbf{25.1}, \textbf{46.4}, \textbf{55.5}] \\
Calculus 3 & [17.6, 31.9, 38.9] & [16.6, 33.1, 39.3] & [13.9, 35.2, 44.4] & [12.4, 35.9, 47.2] & [9.3, 29.6, 38.9] & 
[13.8, 35.5, 45.2] & [6.9, 25.0, 30.1] & [11.4, 31.0, 36.6] & [20.8, 43.1, 49.1] & [\textbf{23.1}, \textbf{48.3}, \textbf{56.9}] \\
Intro. Statistics & [13.4, 36.6, 48.8] & [16.9, 31.0, 41.5] & [17.1, 43.9, 52.4] & [12.0, 44.4, 54.2] & [15.9, 43.9, 
50.0] & [23.2, 50.0, 59.2] & [11.0, 34.1, 45.1] & [8.5, 34.5, 46.5] & [32.9, \textbf{65.9}, \textbf{73.2}] & [\textbf{33.1}, 57.7, 71.8] \\
Business Statistics & [13.3, 33.1, 42.5] & [18.1, 39.1, 44.2] & [13.8, 35.9, 44.2] & [15.3, 41.9, 51.2] & [11.6, 30.4, 43.1] & [18.6, 38.1, 48.4] & [6.1, 23.2, 35.4] & [7.0, 30.2, 39.1] & [27.1, 54.1, 63.0] & [\textbf{29.8}, \textbf{60.9}, \textbf{67.4}] \\
Statistics & [15.3, 40.8, 50.0] & [20.0, 36.1, 43.2] & [20.4, 43.9, 52.0] & [18.1, 42.6, 50.3] & [16.3, 42.9, 54.1] & [21.3, 43.9, 53.5] & [10.2, 35.7, 45.9] & [12.3, 36.1, 45.8] & [28.6, \textbf{60.2}, \textbf{71.4}] & [\textbf{30.3}, 56.8, 65.2] \\
Contemporary Math & [16.3, 40.8, 49.5] & [20.2, 45.4, 55.1] & [18.9, 45.3, 56.8] & [22.0, 53.1, 66.9] & [15.8, 41.6, 
55.5] & [26.4, 51.4, 58.5] & [8.7, 31.6, 37.9] & [13.3, 40.7, 48.6] & [21.8, 49.2, 61.1] & [\textbf{29.4}, \textbf{60.2}, \textbf{71.4}] \\
\hline
Math Avg, & [13.1, 32.4, 41.3] & [14.4, 34.9, 43.0] & [13.6, 35.3, 45.0] & [14.3, 38.7, 49.1] & [12.2, 31.7, 41.8] & [16.3, 37.4, 46.6] & [6.9, 24.9, 33.0] & [8.7, 29.6, 37.5] & [20.7, 46.1, 55.2] & [\textbf{24.6}, \textbf{50.5}, \textbf{59.9}] \\

\hline
\hline
Concepts of Biology & [11.9, 25.7, 31.4] & [13.5, 27.9, 32.8] & [13.3, 35.0, 44.1] & [17.5, 43.4, 52.1] & [14.0, 32.7, 40.3] & [20.1, 41.4, 49.8] & [6.3, 23.9, 31.0] & [11.5, 31.1, 39.7] & [25.5, 52.0, 62.7] & [\textbf{31.7}, \textbf{62.5}, \textbf{71.6}] \\
Biology & [8.2, 18.9, 22.6] & [10.0, 21.6, 25.5] & [8.5, 24.5, 31.8] & [11.9, 32.7, 41.1] & [10.0, 23.6, 30.4] & [17.7, 35.8, 42.4] & [4.3, 17.1, 22.1] & [9.7, 28.8, 36.1] & [18.4, 41.1, 49.2] & [\textbf{26.8}, \textbf{53.4}, \textbf{62.0}] \\
Microbiology & [4.0, 9.0, 11.6] & [4.3, 10.8, 13.7] & [4.1, 11.5, 16.8] & [4.6, 14.7, 20.9] & [5.5, 16.1, 22.3] & [9.8, 23.4, 30.2] & [2.1, 11.1, 16.4] & [3.8, 15.3, 21.4] & [13.6, 31.4, 40.3] & [\textbf{17.7}, \textbf{38.6}, \textbf{47.9}] \\
Chemistry Atoms First & [13.1, 31.2, 38.2] & [14.8, 36.1, 41.7] & [12.5, 35.5, 44.5] & [17.1, 43.2, 53.9] & [12.1, 35.0, 45.0] & [21.9, 46.8, 55.3] & [8.1, 26.0, 35.7] & [15.2, 38.9, 48.8] & [19.0, 44.9, 54.1] & [\textbf{27.1}, \textbf{55.7}, \textbf{63.6}] \\
Chemistry & [42.1, 63.2, 73.7] & [37.5, 56.2, 66.7] & [36.8, 63.2, 73.7] & [37.5, 64.6, 70.8] & [36.8, 68.4, \textbf{86.8}] & [41.7, \textbf{72.9}, 83.3] & [23.7, 63.2, 76.3] & [27.1, 60.4, 72.9] & [42.1, 63.2, 84.2] & [\textbf{43.8}, 62.5, 79.2] \\
Organic Chemistry & [11.2, 22.5, 25.1] & [13.0, 21.7, 26.5] & [10.6, 30.6, 39.7] & [15.1, 39.1, 47.1] & [12.1, 34.6, 
41.6] & [24.2, 48.0, 53.6] & [7.6, 23.8, 31.4] & [16.2, 34.3, 41.4] & [21.2, 46.9, 54.8] & [\textbf{30.0}, \textbf{54.4}, \textbf{61.8}] \\
Anatomy & [4.8, 11.0, 13.6] & [4.9, 13.8, 16.6] & [5.4, 15.8, 21.2] & [6.9, 23.2, 31.7] & [7.5, 20.1, 26.1] & [13.6, 
31.4, 39.3] & [2.7, 15.5, 21.6] & [6.2, 25.4, 34.2] & [14.7, 36.7, 45.8] & [\textbf{20.5}, \textbf{49.1}, \textbf{59.2}] \\
Astronomy & [13.1, 30.3, 38.4] & [\textbf{16.3}, 33.8, 39.3] & [14.1, 33.6, 42.1] & [15.3, \textbf{37.8}, \textbf{45.8}] & [10.4, 25.4, 34.7] & [14.9, 33.5, 42.8] & [9.5, 24.2, 31.2] & [10.0, 30.3, 38.3] & [9.4, 22.3, 29.3] & [12.7, 29.5, 35.6] \\
College Physics & [10.6, 26.5, 34.0] & [14.0, 31.9, 38.4] & [13.0, 29.2, 39.0] & [17.0, 37.2, 48.0] & [10.6, 29.8, 37.9] & [17.0, 39.2, 47.3] & [6.0, 21.3, 29.0] & [7.9, 29.5, 38.4] & [17.9, 41.7, 51.4] & [\textbf{23.9}, \textbf{52.4}, \textbf{62.9}] \\
Physics & [18.0, 35.2, 44.2] & [17.8, 36.3, 45.4] & [18.3, 37.2, 46.8] & [17.1, 41.4, 50.4] & [17.2, 36.9, 46.2] & [20.7, 41.7, 51.1] & [7.9, 27.9, 38.4] & [10.1, 34.0, 44.2] & [22.1, 49.4, 57.9] & [\textbf{23.8}, \textbf{52.6}, \textbf{62.0}] \\
Physics 1 & [11.8, 27.8, 33.8] & [12.1, 30.0, 36.7] & [11.6, 29.6, 39.7] & [11.9, 31.8, 40.5] & [11.8, 29.6, 39.0] & 
[13.4, 34.2, 42.7] & [7.9, 21.0, 27.6] & [8.2, 26.1, 32.5] & [14.3, 38.1, 44.7] & [\textbf{17.3}, \textbf{41.9}, \textbf{49.1}] \\
Physics 2 & [13.8, 28.3, 34.4] & [15.3, 28.8, 34.6] & [15.0, 33.8, 42.9] & [16.6, 37.4, 45.4] & [16.2, 31.6, 41.7] & 
[19.8, 40.6, 49.2] & [8.7, 26.9, 33.8] & [12.1, 33.3, 41.7] & [19.0, 42.5, 50.8] & [\textbf{25.2}, \textbf{49.0}, \textbf{55.1}] \\
Physics 3 & [14.4, 29.2, 36.3] & [17.5, 32.5, 38.3] & [14.1, 33.6, 43.3] & [17.7, 39.7, 48.2] & [13.0, 33.0, 39.4] & 
[19.8, 41.9, 50.3] & [8.5, 25.8, 34.7] & [11.8, 34.4, 42.2] & [22.9, 44.4, 52.0] & [\textbf{30.7}, \textbf{51.1}, \textbf{58.3}] \\
\hline
Science Avg, & [13.6, 27.6, 33.6] & [14.7, 29.3, 35.1] & [13.6, 31.8, 40.4] & [15.9, 37.4, 45.8] & [13.6, 32.1, 40.9] & [19.6, 40.8, 49.0] & [7.9, 25.2, 33.0] & [11.5, 32.4, 40.9] & [20.0, 42.7, 52.1] & [\textbf{25.5}, \textbf{50.2}, \textbf{59.1}] \\

\hline
\hline
U.S. History & [19.4, 33.5, 39.4] & [23.7, 40.7, 45.2] & [23.5, 43.5, 51.1] & [\textbf{31.1}, \textbf{53.3}, \textbf{60.6}] & [16.7, 30.2, 37.4] & [26.1, 43.5, 51.5] & [13.1, 25.4, 32.0] & [19.8, 36.7, 43.3] & [7.8, 14.3, 20.6] & [14.4, 27.0, 32.8] \\
Writing & [16.4, 29.9, 37.5] & [14.8, 29.4, 36.9] & [16.4, 31.6, 41.0] & [15.8, 32.8, 41.7] & [18.9, 34.2, 43.3] & [\textbf{21.1}, \textbf{39.1}, \textbf{48.5}] & [8.7, 20.5, 26.4] & [9.7, 23.9, 31.5] & [9.8, 21.4, 27.9] & [11.0, 26.5, 34.2] \\
Philosophy & [17.2, 29.3, 35.0] & [18.5, 32.2, 38.4] & [17.6, 33.1, 41.8] & [19.8, \textbf{42.1}, \textbf{52.3}] & [15.7, 29.5, 37.3] & [\textbf{22.3}, 38.2, 46.4] & [12.1, 25.5, 32.9] & [17.6, 37.6, 46.0] & [9.0, 20.7, 27.3] & [13.8, 30.0, 38.0] \\
World History 1 & [15.7, 28.3, 33.7] & [17.5, 30.7, 36.1] & [16.0, 30.9, 38.3] & [\textbf{18.3}, \textbf{35.6}, \textbf{43.3}] & [9.1, 21.2, 27.0] & [13.6, 27.6, 33.8] & [8.0, 22.1, 29.6] & [11.4, 29.1, 37.0] & [2.8, 8.5, 12.0] & [4.4, 12.8, 17.0] \\
World History 2 & [24.8, 42.9, 50.5] & [27.3, 47.1, 53.9] & [25.1, 46.7, 55.6] & [\textbf{27.4}, \textbf{50.8}, \textbf{60.2}] & [20.3, 37.3, 45.5] & [24.1, 45.2, 53.3] & [15.5, 35.0, 44.3] & [19.2, 41.9, 51.0] & [8.4, 18.7, 24.5] & [9.8, 23.1, 29.9] \\
\hline

Humanities Avg, & [18.7, 32.8, 39.2] & [20.4, 36.0, 42.1] & [19.7, 37.2, 45.6] & [\textbf{22.5}, \textbf{42.9}, \textbf{51.6}] & [16.1, 30.5, 38.1] & [21.4, 38.7, 46.7] & [11.5, 25.7, 33.0] & [15.5, 33.8, 41.8] & [7.6, 16.7, 22.5] 
& [10.7, 23.9, 30.4] \\

\hline

\hline
Intro. to Business & [12.5, 25.2, 30.3] & [13.8, 27.5, 32.7] & [11.9, 28.1, 35.4] & [13.1, 29.8, 37.2] & [17.9, 33.6, 41.4] & [\textbf{22.9}, \textbf{39.7}, \textbf{45.9}] & [5.3, 14.6, 18.6] & [8.6, 20.6, 25.5] & [8.1, 19.4, 25.0] & 
[14.0, 28.3, 34.8] \\
Financial Accounting & [12.3, 31.4, 38.0] & [13.4, 35.4, 43.0] & [11.5, 35.3, 43.0] & [14.6, 43.6, 52.7] & [17.6, 44.4, 55.8] & [\textbf{28.2}, \textbf{52.7}, \textbf{61.2}] & [6.0, 20.2, 28.4] & [12.1, 35.2, 42.8] & [10.8, 28.4, 37.8] & [18.0, 43.0, 51.3] \\
Managarial Accounting & [13.2, 32.7, 41.5] & [16.8, 41.0, 47.7] & [13.4, 34.9, 47.3] & [14.1, 45.7, 55.6] & [21.0, 47.6, 59.7] & [\textbf{27.7}, \textbf{58.8}, \textbf{69.6}] & [8.6, 25.1, 34.4] & [14.1, 38.3, 48.6] & [15.7, 37.0, 43.0] & [23.2, 49.4, 59.0] \\
Business Ethics & [20.1, 34.1, 40.8] & [21.0, 37.6, 44.7] & [23.2, 41.9, 49.7] & [23.7, 47.2, 51.8] & [24.6, 48.3, 58.1] & [\textbf{36.4}, \textbf{56.1}, \textbf{62.9}] & [11.5, 24.6, 34.9] & [16.7, 36.4, 44.9] & [17.3, 38.0, 46.4] & 
[28.8, 47.0, 54.8] \\
Org. Behavior & [10.0, 22.4, 27.7] & [13.2, 28.5, 34.4] & [9.3, 22.9, 30.1] & [13.4, 30.9, 38.7] & [13.9, 31.2, 41.7] & [\textbf{30.4}, 47.6, 55.4] & [4.8, 16.9, 21.5] & [12.6, 32.7, 39.0] & [13.2, 27.5, 37.7] & [27.9, \textbf{48.4}, 
\textbf{56.3}] \\
Finance & [11.0, 25.1, 34.6] & [16.5, 31.4, 38.9] & [10.7, 28.5, 37.8] & [15.4, 34.0, 44.5] & [19.3, 41.6, 51.6] & [\textbf{25.1}, \textbf{47.1}, \textbf{56.3}] & [5.3, 19.0, 27.9] & [9.5, 28.6, 35.4] & [13.0, 29.8, 36.9] & [18.4, 38.0, 45.0] \\
Business Law & [19.7, 38.5, 46.2] & [21.1, 39.6, 47.5] & [20.1, 44.6, 51.3] & [21.4, 45.7, 56.0] & [23.6, 49.0, 56.7] & [\textbf{30.8}, \textbf{52.8}, \textbf{63.3}] & [9.9, 27.7, 36.6] & [15.2, 34.0, 44.0] & [15.9, 32.8, 41.1] & [19.6, 44.9, 52.8] \\
Intellectual Property & [18.2, 45.5, 59.6] & [22.7, 46.2, 55.5] & [18.2, 45.5, 61.6] & [21.8, 45.4, 57.1] & [21.2, 49.5, \textbf{65.7}] & [\textbf{23.5}, \textbf{49.6}, 63.0] & [7.1, 34.3, 46.5] & [9.2, 37.8, 50.4] & [9.1, 36.4, 54.5] & [17.6, 42.9, 54.6] \\
Marketing & [8.3, 19.3, 23.5] & [9.3, 20.6, 24.9] & [9.4, 22.5, 29.4] & [9.6, 22.8, 28.2] & [16.6, 31.3, 37.6] & [\textbf{23.8}, \textbf{39.0}, \textbf{44.0}] & [4.6, 12.6, 17.3] & [7.6, 19.1, 22.7] & [7.5, 16.9, 22.0] & [14.8, 26.7, 
32.0] \\
Management & [18.7, 33.7, 40.3] & [20.9, 38.0, 45.8] & [18.4, 37.5, 45.4] & [22.0, 44.0, 50.0] & [24.1, 43.2, 54.3] & [\textbf{41.4}, \textbf{59.2}, \textbf{64.9}] & [11.7, 30.2, 37.8] & [21.7, 44.2, 50.3] & [20.0, 39.0, 49.5] & [35.6, 55.8, 64.4] \\
Economics & [11.8, 33.1, 41.3] & [14.7, 37.3, 47.3] & [13.3, 34.6, 44.7] & [15.7, 40.7, 53.2] & [16.0, 38.0, 47.4] & 
[\textbf{23.7}, \textbf{50.4}, 57.9] & [5.0, 21.8, 29.1] & [8.3, 32.0, 39.7] & [14.8, 36.5, 46.5] & [21.1, 48.0, \textbf{59.6}] \\
Macroeconomics & [24.1, 63.1, 70.9] & [27.7, 66.7, 74.5] & [17.7, 59.6, 71.6] & [24.1, 63.1, 77.3] & [27.0, 59.6, 67.4] & [\textbf{34.0}, 66.7, 78.0] & [7.8, 42.6, 53.9] & [16.3, 48.9, 63.1] & [30.5, 62.4, 73.0] & [33.3, \textbf{72.3}, \textbf{80.1}] \\
Microeconomics & [30.9, 60.5, 72.8] & [30.0, 63.7, 72.5] & [28.4, 65.4, 71.6] & [28.7, 68.8, 73.8] & [33.3, 59.3, 75.3] & [37.5, 73.8, 78.8] & [16.0, 50.6, 60.5] & [26.2, 62.5, 71.2] & [35.8, 66.7, 84.0] & [\textbf{42.5}, \textbf{80.0}, \textbf{86.2}] \\
Entrepreneurship & [9.8, 24.1, 29.3] & [11.3, 27.8, 33.8] & [10.7, 25.9, 33.4] & [10.8, 28.4, 34.9] & [16.7, 35.1, 41.5] & [\textbf{25.1}, \textbf{43.8}, \textbf{49.7}] & [5.4, 15.9, 20.8] & [8.1, 24.1, 30.9] & [8.0, 20.4, 27.1] & [14.9, 29.8, 36.7] \\
\hline

Business Avg,& [15.8, 34.9, 42.6] & [18.0, 38.7, 45.9] & [15.4, 37.7, 46.6] & [17.7, 42.1, 50.8] & [20.9, 43.7, 53.9] & [\textbf{29.3}, \textbf{52.7}, \textbf{60.8}] & [7.8, 25.4, 33.4] & [13.3, 35.3, 43.5] & [15.7, 35.1, 44.6] & 
[23.6, 46.8, 54.8] \\

\hline
\hline
Nutrition & [7.8, 17.0, 21.7] & [8.2, 18.1, 23.5] & [8.1, 18.3, 24.3] & [8.3, 20.1, 27.2] & [10.2, 26.8, 35.3] & [13.7, 31.6, 40.1] & [2.5, 10.3, 15.7] & [3.9, 13.8, 19.4] & [18.3, 39.1, 50.3] & [\textbf{20.2}, \textbf{41.3}, \textbf{51.5}] \\
\hline

Nursing Avg,& [7.8, 17.0, 21.7] & [8.2, 18.1, 23.5] & [8.1, 18.3, 24.3] & [8.3, 20.1, 27.2] & [10.2, 26.8, 35.3] 
& [13.7, 31.6, 40.1] & [2.5, 10.3, 15.7] & [3.9, 13.8, 19.4] & [18.3, 39.1, 50.3] & [\textbf{20.2}, \textbf{41.3}, \textbf{51.5}] \\

\hline

\hline
Python Programming & [8.8, 17.7, 22.3] & [9.2, 16.7, 21.8] & [9.4, 23.1, 27.5] & [11.2, 22.8, 28.2] & [17.7, 34.0, 43.6] & [\textbf{19.2}, \textbf{38.6}, \textbf{50.5}] & [3.6, 14.0, 22.3] & [4.9, 14.1, 19.2] & [15.1, 29.1, 33.0] & [14.8, 28.9, 34.2] \\
Workplace Software & [7.9, 20.1, 25.5] & [9.8, 25.8, 31.6] & [8.1, 20.8, 28.9] & [9.6, 27.2, 35.0] & [16.9, 35.9, 44.2] & [\textbf{22.3}, \textbf{44.6}, \textbf{52.4}] & [3.9, 13.2, 18.3] & [5.3, 19.1, 25.8] & [8.8, 22.1, 29.0] & [10.2, 30.2, 38.3] \\
\hline

C.S Avg,& [8.4, 18.9, 23.9] & [9.5, 21.2, 26.7] & [8.8, 22.0, 28.2] & [10.4, 25.0, 31.6] & [17.3, 35.0, 43.9] & [\textbf{20.8}, \textbf{41.6}, \textbf{51.5}] & [3.8, 13.6, 20.3] & [5.1, 16.6, 22.5] & [11.9, 25.6, 31.0] & [12.5, 29.5, 36.2] \\

\hline

\hline
American Government & [17.7, 27.8, 31.7] & [19.9, 35.9, 40.5] & [18.5, 30.6, 35.0] & [19.3, 33.3, 38.8] & [17.3, 29.9, 36.6] & [\textbf{37.2}, \textbf{49.8}, \textbf{54.8}] & [11.3, 20.2, 24.4] & [19.7, 38.1, 43.3] & [5.9, 14.5, 20.3] & [26.4, 37.2, 42.7] \\
Anthropology & [11.7, 23.5, 29.8] & [12.9, 27.3, 33.8] & [13.3, 28.7, 35.1] & [15.0, 35.2, \textbf{43.1}] & [12.4, 25.2, 31.9] & [\textbf{19.6}, \textbf{35.3}, 40.8] & [8.0, 20.5, 26.7] & [11.5, 29.7, 36.6] & [7.6, 18.0, 23.5] & [12.8, 27.8, 33.7] \\
Political Science & [14.4, 25.1, 30.7] & [15.9, 34.0, 40.4] & [14.7, 28.3, 34.8] & [14.7, 31.0, 38.2] & [18.7, 33.2, 
38.9] & [\textbf{36.6}, \textbf{50.4}, \textbf{55.4}] & [9.0, 20.4, 26.2] & [17.4, 38.3, 44.1] & [9.6, 20.4, 25.9] & 
[29.2, 40.9, 45.0] \\
Psychology & [14.8, 28.2, 34.3] & [16.0, 30.8, 37.0] & [15.6, 32.6, 41.2] & [18.0, 40.8, 47.7] & [17.8, 37.4, 46.0] & [25.9, 46.9, 54.2] & [5.9, 19.1, 27.0] & [11.2, 31.6, 40.9] & [20.7, 40.7, 49.0] & [\textbf{28.7}, \textbf{52.2}, \textbf{59.4}] \\
Sociology & [19.7, 44.0, 51.3] & [20.7, 52.8, 60.4] & [19.7, 46.8, 57.3] & [24.4, 58.5, 66.9] & [27.0, 50.6, 61.4] & 
[\textbf{37.6}, \textbf{64.1}, \textbf{70.9}] & [8.6, 26.8, 36.0] & [16.5, 46.1, 55.2] & [15.9, 39.0, 48.5] & [28.0, 
55.9, 63.9] \\
\hline

Social Sci. Avg,& [15.7, 29.7, 35.6] & [17.1, 36.2, 42.4] & [16.4, 33.4, 40.7] & [18.3, 39.8, 46.9] & [18.6, 
35.3, 43.0] & [\textbf{31.4}, \textbf{49.3}, \textbf{55.2}] & [8.6, 21.4, 28.1] & [15.3, 36.8, 44.0] & [11.9, 26.5, 33.4] & [25.0, 42.8, 48.9] \\

\hline

\hline
College Success & [33.3, 51.9, 66.7] & [39.7, 58.9, 65.8] & [37.0, 57.4, 68.5] & [41.1, 61.6, 65.8] & [38.9, 72.2, 81.5] & [\textbf{52.1}, \textbf{76.7}, \textbf{86.3}] & [25.9, 48.1, 61.1] & [23.3, 50.7, 63.0] & [25.9, 55.6, 72.2] & 
[41.1, 65.8, 74.0] \\
College Success Concise & [40.4, 57.9, 59.6] & [37.9, 53.4, 62.1] & [36.8, 59.6, 68.4] & [41.4, 65.5, 69.0] & [45.6, 
70.2, 84.2] & [\textbf{53.4}, \textbf{75.9}, \textbf{86.2}] & [17.5, 38.6, 57.9] & [29.3, 55.2, 69.0] & [26.3, 59.6, 
66.7] & [31.0, 62.1, 70.7] \\

\hline
Domain College Success  & [36.8, 54.9, 63.2] & [38.8, 56.1, 64.0] & [36.9, 58.5, 68.5] & [41.2, 63.5, 67.4] & [42.2, 
71.2, 82.8] & [\textbf{52.8}, \textbf{76.3}, \textbf{86.2}] & [21.7, 43.4, 59.5] & [26.3, 53.0, 66.0] & [26.1, 57.6, 
69.5] & [36.0, 64.0, 72.3] \\

\hline
\hline
Overall & [15.2, 31.7, 38.9] & [16.8, 34.7, 41.6] & [15.4, 35.1, 43.8] & [17.4, 39.8, 48.4] & [16.9, 36.5, 45.9] & [\textbf{23.7}, 44.8, 53.1] & [8.3, 24.9, 32.9] & [12.2, 32.9, 41.0] & [17.1, 37.6, 46.4] & [23.2, \textbf{45.9}, \textbf{54.2}] 
\\
\hline
        
\end{tabular}
\caption{\label{causal-lms} Masked models' accuracies (percentages) \textbf{on the English portion of the dataset}. Results are shown as [top1, top5, top10]. Books that are also in Polish are marked with $\textcolor{red}\diamond$, where books that are also in Spanish are marked with $\textcolor{purple}\star$, and their results can be seen in Tables T1, T2. S=sentence-level prompts; P=paragraph-level prompts.}
\end{table*}

==> results_table.tex <==
\begin{table*}
\centering
\setlength{\tabcolsep}{1.5pt}
\small
\begin{tabular}{ll|llll|lllll}
\hline
\multicolumn{1}{c}{\textbf{Domain}} & \multicolumn{1}{c|}{\textbf{Subdomain}} & \multicolumn{4}{c|}{\textbf{Causal LMs}} & \multicolumn{5}{c}{\textbf{Masked LMs}} \\
& & \textbf{Bloom} & \textbf{Mistral} & \textbf{Llama2} & \textbf{Llama3} & \textbf{BERT} & \textbf{DistilBERT} & \textbf{XLM-RoBERTa} & \textbf{mBERT} & \textbf{SciBERT} \\
\hline


\multirow{5}{*}{Math} 
        & Prealgebra & - & - & - & - & - & - & - & - & - \\
        
        & Elementary Algebra & - & - & - & - & - & - & - & - & - \\
        
        & Intermediate Algebra & - & - & - & - & - & - & - & - & - \\
        
        & College Algebra & - & - & - & - & - & - & - & - & - \\
        
        & Trigonometry & - & - & - & - & - & - & - & - & - \\
        
        & Precalculus $\textcolor{purple}\star$ & - & - & - & - & - & - & - & - & - \\
        
        & Calculus I $\textcolor{purple}\star$ & - & - & - & - & - & - & - & - & - \\
        
        & Calculus II $\textcolor{purple}\star$ & - & - & - & - & - & - & - & - & - \\
    
        & Calculus III $\textcolor{purple}\star$ & - & - & - & - & - & - & - & - & - \\

        & Intro. Statistics & - & - & - & - & - & - & - & - & - \\

        & Business Statistics $\textcolor{purple}\star$ & - & - & - & - & - & - & - & - & - \\
        
        & Statistics & - & - & - & - & - & - & - & - & - \\
        
        & Contemporary Math & - & - & - & - & - & - & - & - & - \\
        \hline

\multirow{5}{*}{Science} 
        & Concepts of Biology & - & - & - & - & - & - & - & - & - \\
        
        & Biology & - & - & - & - & - & - & - & - & - \\

        & Microbiology & - & - & - & - & - & - & - & - & - \\
        
        & Chemistry Atoms First & - & - & - & - & - & - & - & - & - \\
        
        & Chemistry $\textcolor{purple}\star$ & - & - & - & - & - & - & - & - & - \\
        
        & Organic Chemistry & - & - & - & - & - & - & - & - & - \\
    
        & Anatomy & - & - & - & - & - & - & - & - & - \\
        
        & Astronomy & - & - & - & - & - & - & - & - & - \\

        & College Physics & - & - & - & - & - & - & - & - & - \\

        & Physics & - & - & - & - & - & - & - & - & - \\
        
        & Physics I $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & - & - & - & - & - & - & - & - & - \\
        
        & Physics II $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & - & - & - & - & - & - & - & - & - \\
        
        & Physics III $\textcolor{red}\diamond$ $\textcolor{purple}\star$ & - & - & - & - & - & - & - & - & - \\
        \hline
        
\multirow{5}{*}{Humanities} 
        & U.S. History & - & - & - & - & - & - & - & - & - \\
        & Writing & - & - & - & - & - & - & - & - & - \\
        & Philosophy & - & - & - & - & - & - & - & - & - \\
        & World History I & - & - & - & - & - & - & - & - & - \\
        & World History II & - & - & - & - & - & - & - & - & - \\
        \hline

\multirow{5}{*}{Business} 
        & Intro. to Business & - & - & - & - & - & - & - & - & - \\
        
        & Accounting I & - & - & - & - & - & - & - & - & - \\
        
        & Accounting II & - & - & - & - & - & - & - & - & - \\
        
        & Business Ethics & - & - & - & - & - & - & - & - & - \\
        
        & Org. Behavior & - & - & - & - & - & - & - & - & - \\
        
        & Finance & - & - & - & - & - & - & - & - & - \\
        
        & Business Law & - & - & - & - & - & - & - & - & - \\
        
        & Intellectual Property & - & - & - & - & - & - & - & - & - \\
    
        & Marketing & - & - & - & - & - & - & - & - & - \\
        
        & Management & - & - & - & - & - & - & - & - & - \\
        
        & Economics & - & - & - & - & - & - & - & - & - \\
        
        & Macroeconomics $\textcolor{red}\diamond$ & - & - & - & - & - & - & - & - & - \\
        
        & Microeconomics $\textcolor{red}\diamond$ & - & - & - & - & - & - & - & - & - \\
        
        & Entrepeneurship & - & - & - & - & - & - & - & - & - \\
        \hline

\multirow{1}{*}{Nursing}    
        & Nutrition & - & - & - & - & - & - & - & - & - \\
        \hline

\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Computer \\ Science\end{tabular}} & Python Programming & - & - & - & - & - & - & - & - & - \\ 

& Workplace Software & - & - & - & - & - & - & - & - & - \\

        \hline

\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Social \\ Sciences\end{tabular}} & American Government & - & - & - & - & - & - & - & - & - \\
        & Anthropology & - & - & - & - & - & - & - & - & - \\
        & Political Science & - & - & - & - & - & - & - & - & - \\
        & Psychology $\textcolor{red}\diamond$ & - & - & - & - & - & - & - & - & - \\
        & Sociology & - & - & - & - & - & - & - & - & - \\
        \hline

\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}College \\ Success\end{tabular}}    
        & College Success & - & - & - & - & - & - & - & - & - \\
        & College Success Concise & - & - & - & - & - & - & - & - & - \\
        \hline
\end{tabular}
\caption{\label{citation-guide}
Models' accuracies (percentages). Books that are also in Polish are marked with $\textcolor{red}\diamond$, where books that are also in Spanish are marked with $\textcolor{purple}\star$. }
\end{table*}


